Intention-Conditioned Long-Term Human Egocentric Action Forecasting

To anticipate how a human would act in the future, it is essential to understand the human intention since it guides the human towards a certain goal. In this paper, we propose a hierarchical architecture which assumes a sequence of human action (low-level) can be driven from the human intention (high-level). Based on this, we deal with Long-Term Action Anticipation task in egocentric videos. Our framework first extracts two level of human information over the N observed videos human actions through a Hierarchical Multi-task MLP Mixer (H3M). Then, we condition the uncertainty of the future through an Intention-Conditioned Variational Auto-Encoder (I-CVAE) that generates K stable predictions of the next Z=20 actions that the observed human might perform. By leveraging human intention as high-level information, we claim that our model is able to anticipate more time-consistent actions in the long-term, thus improving the results over baseline methods in EGO4D Challenge. This work ranked first in both CVPR@2022 and ECVV@2022 EGO4D LTA Challenge by providing more plausible anticipated sequences, improving the anticipation of nouns and overall actions. Webpage: https://evm7.github.io/icvae-page/

==> tables/ICVAE_strategy.tex <==
\begin{table}
\centering
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{cccc|cc}
\multicolumn{4}{c|}{\textbf{Conditions}} & \multicolumn{2}{c}{\textbf{ED@20}} \\  \hline
\multirow{2}{*}{\textbf{Embedding}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Action\\ Space\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Focal\\ Loss\end{tabular}}} & \multirow{2}{*}{\textbf{Noise}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Verbs\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}} Nouns\end{tabular}}} \\
 &  &  &  &  &  \\
  \hline
Learnable       & \cmark & \cmark  & 0.3 & {\ul 0.697} & {\ul 0.587} \\
Learnable       & \xmark & \cmark  & 0.3 & 0.704                & \textbf{0.585}       \\
Learnable       & \xmark & \cmark  & 0.4 & \textbf{0.696}       & 0.593                \\
Learnable       & \xmark & \cmark  & 0.2 & 0.708                & 0.587                \\
%Learnable       & \xmark & \cmark  & 0.2 & 0.703                & 0.599                \\
Learnable       & \cmark  & \xmark & 0.0   & 0.709                & 0.594                \\
S-BERT  & \xmark & \cmark  & 0.1 & 0.716                & 0.6096               \\
FT S-BERT & \xmark & \cmark  & 0.1 & 0.716                & 0.612               
\end{tabular}
}
\caption{Strategy analysis of I-CVAE. The first strategy reported the best results in LTA challenge. Embedding: how the observed verb-noun pairs are projected into the action representation: the embedded layer can be trained from scratch (learnable) or from the pre-trained S-BERT language model \cite{sbert} (FT: Fine-tuned). Action space: whether to project the verb-noun action pair in the same representation space. Focal loss \cite{focal_loss}: whether to tackle imbalance dataset. Noise: percentage of manually corrupted actions in the observed sequence.}
\label{tab:ICVAE_strategy}
\end{table}
